Data-driven Optimization and Transfer Learning for Cellular Network Antenna Configurations

We propose a data-driven approach for large-scale cellular network optimization, using a production cellular network in London as a case study and employing Sionna ray tracing for site-specific channel propagation modeling. We optimize base station antenna tilts and half-power beamwidths, resulting in more than double the 10\%-worst user rates compared to a 3GPP baseline. In scenarios involving aerial users, we identify configurations that increase their median rates fivefold without compromising ground user performance. We further demonstrate the efficacy of model generalization through transfer learning, leveraging available data from a scenario source to predict the optimal solution for a scenario target within a similar number of iterations, without requiring a new initial dataset, and with a negligible performance loss.

==> XX_Results.tex <==
\section{Numerical Results and Conclusion}

\subsubsection*{Performance of HD-BO} Fig.~\ref{fig:SINR_CDFs_tilts_vHPBW} shows the cumulative distribution function (CDF) of the perceived SINR when optimizing the cellular network for GUEs and UAVs with equal weight ($\lambda = 0.5$). The figure shows that for the baseline configuration, 80\% of the UAVs experience SINRs below \mbox{-5\,dB} and can thus be regarded as being in outage. The joint antenna tilt and HPBW optimization through TuRBO improves the UAV SINR, with median gains of around 7\,dB, reducing the percentage of UAVs in outage from 80\% to less than 2\%. This UAV performance improvement does not correspond to a severe GUE performance degradation. 

\begin{figure}
\centering
\includegraphics[width=\figwidth]{Figures/2024_08_05_RD_TL_Corr_150m_Rates_CDFs.eps}
\caption{Rates for UAVs and GUEs when the network is optimized for both and for an all-downtilt baseline.}
\label{fig:SINR_CDFs_tilts_vHPBW}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=\figwidth]{Figures/2024_08_05_RD_TL_Corr_150m_Config.eps}
\caption{Optimized tilts and HPBW for $\lambda = 0.5$. Green circles and blue diamonds denote BSs serving GUEs and UAVs, respectively.}
\label{fig:Opt_Tilts_vHPBW_config_TuRBO}
\end{figure}

\subsubsection*{Transfer Learning with HD-BO} 
The adoption of an optimization framework in a commercial network hinges on its consistent performance across various scenarios. We present the generalization capabilities of the HD-BO framework across different scenarios (i.e., UE distributions) within the context of \emph{scenario-specific transfer learning}. Transfer learning in optimization leverages knowledge or data from a previously solved problem (\emph{source}) to accelerate the solution of a new, related problem (\emph{target}). This can be particularly advantageous when data collection is costly or time-consuming.  

Figure~\ref{fig:LT_conv_50m_150m} illustrates the convergence of scenario-specific transfer learning using HD-BO, showing the best observed objective at each iteration $n$. Three evaluations were conducted, varying the initial dataset's dependency on the scenario target: 100\% scenario target (no transfer learning), 50\%, and 0\% (full transfer learning). Notably, with a 50\% reliance on the target's initial dataset, convergence occurs within a similar number of iterations, indicating that resources can be conserved when data sampling for the scenario target is costly. Even without prior knowledge of the target (initial dataset solely from the scenario source), performance declines by only a marginal 1\%. 




